Compilation of Commit Changes within Java Source Code Repositories

Java applications include third-party dependencies as bytecode. To keep these applications secure, researchers have proposed tools to re-identify dependencies that contain known vulnerabilities. Yet, to allow such re-identification, one must obtain, for each vulnerability patch, the bytecode fixing the respective vulnerability at first. Such patches for dependencies are curated in databases in the form of fix-commits. But fixcommits are in source code, and automatically compiling whole Java projects to bytecode is notoriously hard, particularly for non-current versions of the code. In this paper, we thus propose JESS, an approach that largely avoids this problem by compiling solely the relevant code that was modified within a given commit. JESS reduces the code, retaining only those parts that the committed change references. To avoid name-resolution errors, JESS automatically infers stubs for references to entities that are unavailable to the compiler. A challenge is here that, to facilitate the above mentioned reidentification, JESS must seek to produce bytecode that is almost identical to the bytecode which one would obtain by a successful compilation of the full project. An evaluation on 347 GitHub projects shows that JESS is able to compile, in isolation, 72% of methods and constructors, of which 89% have bytecode equal to the original one. Furthermore, on the Project KB database of fix-commits, in which only 8% of files modified within the commits can be compiled with the provided build scripts, JESS is able to compile 73% of all files that these commits modify.

==> sections/concept/parsing.tex <==
\subsection{Parsing}
\label{subsec:parsing}
In its initial phase, \jess receives a target file containing the class members for compilation, a specification of which members to target and the available parts of the code base as input.
%As previously mentioned, \jess is able to compile all types of class members like methods, constructors, fields and initializers, even when they are part of inner classes. \wolf{IMHO this sentence is redundant/doesn't add anything here.}
As previously mentioned, we describe the process for compiling one target method, as other class members are handled analogously.

%For compiling class members, \jess provides multiple options.
%Targeted methods and constructors can be addressed by specifying their uniquely identifying signatures.
%For initializers and fields, \jess provides two separate options.
%The Java compiler compiles static fields and initializers into a \texttt{<clinit>} method in the bytecode, which serves the purpose of a class initialization method~\cite{jvmStructure}.
%There exists only a single \texttt{<clinit>} method per class and therefore \jess provides an option that keeps all static fields and initializers of the target file intact.
%Non-static fields and initializers are compiled into all \texttt{<init>} methods within a class, which serve the purpose of instance initialization methods~\cite{jvmStructure}.
%Each \texttt{<init>} method in the bytecode represents one constructor within the source code.
%\jess provides an option that keeps all non-static fields and initializers of the target class intact.
%Moreover, this also means, that if the compilation target is a constructor, in turn all non-static fields and initializers within the target class need to be kept intact to obtain the original bytecode.

First \jess parses the target Java file into an Abstract Syntax Tree (AST). 
%which makes it more practical to interact with different kinds of constructs within a class. \wolf{Remove 'representation which makes it more practical to interact with different kinds of constructs within a class.' - common knowledge}
After parsing, \jess marks the method within the target file that has been specified as target for compilation.
There are two types of markings: \textit{Keep-All-Markings} and \textit{Keep-Markings}.
%Keep-All-Markings specify that the marked member should not be altered at all, e.g. when a method is marked with a Keep-All-Marking, the method body is not sliced. 
Keep-All-Markings specify that the marked member should not be altered, for methods and constructors this means the body is not sliced or modified.
%Keep-Markings specify that the signature of the member should be kept, but the content can be sliced, e.g. when a method is marked with a Keep-Marking, its signature is kept intact, but the method body is sliced away. 
Keep-Markings specify that only the signature of the member should be kept e.g. for methods the signature is kept while the body is sliced away.
To keep its body intact, the initial target method is marked with a Keep-All-Marking.

==> sections/concept/resolution.tex <==
\subsection{Resolution}
\label{subsec:resolution}
%During the resolution step, \jess takes the method that has been marked and tries to resolve all references made to other members or types within the provided code base.
%This means that \jess tries to find the corresponding declaration for each reference. 
%\jo{maybe put Parsing and Resolution together. Your Parsing section feels like a small sentences you put before the Resolution}
In the resolution step, \jess at first identifies all parts of the available code base that are relevant for compiling the target method.
By doing so, \jess ensures that, in the next step, the relevant parts are kept, while the parts that are not required for compiling the target method, which would only interfere with the compilation, are removed.
To do so, \jess takes the method that has been marked and tries to find the corresponding declaration for each reference, e.g. field accesses, method invocations or object creations.
Depending on the type of marking, different references are considered.
If a method or constructor is marked with a Keep-All-Marking, every reference within the signature and body has to be resolved.
If a method or constructor is marked with a Keep-Marking, only references within the signature are resolved.
For fields that are marked with a Keep-All-Marking, the type definition and the field initializer need to be resolved.
Otherwise only the type definition is resolved.
The resolved references can e.g.\ include field accesses, method/constructor invocations, object creation expressions or simple type specifications.
Whenever such a reference is detected, the referenced member is marked with a Keep-Marking, indicating that, while its content can be sliced, the signature has to be kept intact.
The referenced members are marked with a Keep-Marking since the Java compiler, to be able to compile the targeted members, generally only requires the corresponding signatures of the referenced types and members.
By slicing away the body of a method that is invoked from within the target method, while keeping its signature in place, \jess minimizes the amount of transitively referenced members, while at the same time obtaining compilable code.
All newly marked members are recursively resolved until all relevant members within the provided code base have been marked.
%Whenever a member has been marked, its declaring class is added to the worklist and needs to be considered for resolution as well.
%The resolution and marking process is repeated until the worklist is empty and all relevant members within the provided code base have been marked.
%\wolf{All marked members are recursively resolved in the available code. Instead of the two previous sentences ?!? } \wolf{The worklist is IMHO an implementation detail - why mention it here?}
Whenever a reference is made to a member that is not part of the available code base, including JAR files, there is nothing that can be marked and essential code parts are missing for the compilation.
Cases like these are handled during the stub generation step, which we explain later. 
Once the resolution process is finished, all marked files are handed to the slicing step. 

%Listings~\ref{lst:classA},~\ref{lst:classB} and~\ref{lst:classC} illustrate an example of how \jess performs the resolution.
%Listing~\ref{lst:classA} shows the target file with the target member being the \texttt{visit} method.
%In the first step of resolution, \jess marks the method with a Keep-All-Marking as the whole method body should be kept intact.
%The numbers next to the markings within the listings indicate the resolution iteration in which the corresponding member has been marked.
%In the next step, \jess resolves all references made from within the \texttt{visit} method.
%In line 9, a new object of class \texttt{B} is created and the constructor \texttt{B(int a)} in line 5 of Listing~\ref{lst:classB} is invoked.
%Due to this invocation, \jess marks the constructor with a Keep-Marking, since the constructor signature needs to be kept intact to compile the target method.
%Furthermore, in line 10 of Listing~\ref{lst:classA}, the \texttt{inc(int a)} method of class \texttt{B} is invoked, which \jess also marks with a Keep-Marking.
%This method invocation receives the field \texttt{num} as argument and therefore \jess marks the field declaration in line 3 of Listing~\ref{lst:classA} with a Keep-Marking.
%There are no further references made from within the target method's body or signature.
%Now \jess looks at all members that have been marked in the previous step.
%Since all added markings are Keep-Markings, only the member signatures are of interest, since their content will be sliced away in the next step anyway.
%The only additional reference can be seen in line 8 of Listing~\ref{lst:classB}. \jo{arent all markers Keep and only the single method you want to compile a Keep all}
%The \texttt{inc} method specifies a return type of \texttt{C}.
%Because of this, a Keep-Marking is added to the class C (cf. line 1 of Listing~\ref{lst:classC}).
%\jo{You could mark the things in the listings that cause the Keep markers. The reason for Keep 3 might be hard to spot}
%%Since there are no further references made from the marked members, \jess stops the resolution process and hands the marked files to the slicing step. \wolf{'and hands the marked files to the slicing step.' kind of redundant because I know this from the paragraph above.}
%
%
%\noindent
%\begin{figure}
%	\begin{minipage}[t]{.29\linewidth}
%		\begin{lstlisting}
%public class A {
%  @Keep // 2
%  int num = D.getNumber();
%  
%  int otherNum = 12;
%
%  @KeepAll // 1
%  public int visit() {
%    B b = new B(23);
%    b.inc(num);
%    return num;
%  }
%}
%		\end{lstlisting}
%		\subcaption{Target file}
%		\label{lst:classA}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[t]{.29\linewidth}
%		\begin{lstlisting}
%public class B {
%  String x = D.getName();
%  
%  @Keep // 2
%  public B(int a) {...}
%
%  @Keep // 2
%  public C inc(int a) 
%  {...}
%
%  public E dec(int a) 
%  {...}
%}
%		\end{lstlisting}
%		\subcaption{Support file 1}
%		\label{lst:classB}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[t]{.29\linewidth}
%		\begin{lstlisting}
%@Keep // 3
%public class C {
%  String city = "London";
%
%  public void visit(F f) {
%    Extern e = new Extern();
%    e.process(f);
%  }
%
%  private String concat() 
%  {...}
%}
%		\end{lstlisting}
%		\subcaption{Support file 2}
%		\label{lst:classC}
%	\end{minipage}
%	\caption{Resolution example}
%	\label{lst:std}
%\end{figure}
